Formally-verified Security against Forgery of Remote Attestation using SSProve

Remote attestation (RA) is the foundation for trusted execution environments in the cloud and trusted device driver onboarding in operating systems. However, RA misses a rigorous mechanized definition of its security properties in one of the strongest models, i.e., the semantic model. Such a mechanization requires the concept of StateSeparating Proofs (SSP). However, SSP was only recently implemented as a foundational framework in the Rocq Prover. Based on this framework, this paper presents the first mechanized formalization of the fundamental security properties of RA. Our Rocq Prover development first defines digital signatures and formally verifies security against forgery in the strong existential attack model. Based on these results, we define RA and reduce the security of RA to the security of digital signatures. Our development provides evidence that the RA protocol is secure against forgery. Additionally, we extend our reasoning to the primitives of RA and reduce their security to the security of the primitives of the digital signatures.

==> src/implementation.tex <==
\section{Implementation}
\label{sec:implement}

%
Our formalization was implemented by a novice user outside the \ssprove community, 
demonstrating the accessibility and usability of the \coq
with \ssprove and the mathematical componenents library MathComp~\cite{mahboubi2021mathematical} for cryptographic formalization.
%
The formal development consists of several components of reasonings, 
each contributing to different parts of our formalization. 
%
%
\begin{table}[b]
    \centering  
    %\begin{minipage}  
    \begin{tabular}{ ||c|c||}
        \hline 
        %\rowcolor{lightgray} Files & Lines of Code \\[0.5ex] 
        \textbf{Reasonings} & \textbf{Lines of Code} \\[0.5ex] 
        \hline
        Signature & 296 \\
        SigProt & 327 \\
        RA & 263 \\
        AttProt & 1470 \\ 
        \hline
        \rowcolor{lightgray} Total & 2356 \\ [1ex] 
        \hline
    \end{tabular}
    \caption{Lines of code for each component}\label{fig:LOC}
    %\end{minipage}
    \end{table}
%
%
Table~\ref{fig:LOC} overviews these components, including 
their respective line counts to show our effort estimate.
%
Our formal development shows that we invested some time in understanding 
the \coq environment and the \ssprove framework for a generalized proof structure.
%
Our efforts highlight \ssprove's modularity and clarity, allowing new users to define, 
verify effectively, and reason about security protocols. 
%

While working with the \ssprove library in the \coq, we explored the 
\emph{swap} tactic, which enables 
reordering operations in probabilistic programs—a key component 
of reasoning in game-based cryptographic proofs.
%
\ssprove only supports \emph{swap}ing pure commands in procedure.
%
We added a more general lemma that allows to swap stateful 
commands for as long as they do not reference the same 
location, i.e., state, contributing it back to the library 
to strengthen its capabilities.
%
We also made several smaller contributions, enhancing the 
library's functionality and clarity.
%
Amongst others, we updated it to the latest version of MathComp.
%
We hope these additions will support and ease the work 
of researchers engaging with \ssprove in the future. 
%

%
The only gap in our development is due to a composition
gap in \ssprove.
%
Our Hypothesis for the functional correctness of the
digitial signature schema $\Sigma$ (Figure~\ref{fig:sigprim:hypo})
has a monadic precondition, i.e., the call to $\Sigma$.\icoq{KeyGen}.
%
This call needs to be monadic because it needs to sample.
%
See our RSA implementation in Section~\ref{sec:rsa} for 
the details.
%
Instantiating this precondition in the indistinguishability 
proof for Theorem~\ref{theo:indist-signature} was not
possible.
%
This is due to the monadic construction that underpins
the relational Hoare Logic in \ssprove.
%
Adding support for such instantiations of facts
is an interesting topic for future research.
%


==> src/implications.tex <==
\section{From Theory to Framework: A Discussion on Indistinguishability for Libraries}
\label{sec:imply}
%
%\begin{minipage}[b]{.67\textwidth}\centering
%\begin{table}[p]
  %\centering
 % \begin{tabular}{ |p{1in}|p{1in}|p{1in}|p{1in}|p{1in}|p{1in}|}
 %   \hline
 %   \rowcolor{lightgray} \textbf{} & \textbf{ElGamal} & \textbf{PRF} & \textbf{KEMDEM} & \textbf{\Sigma protocol} & \textbf{Our Proofs} \\
%    \hline
 %   \textit{No. Lib Procedures} & xxx & aaa & bb & cc & dd \\
 %   \hline
 %   \textit{Ideal Model State} & None & Local & Distribution & Distribution & None \\
 %   \hline
 %   \textit{Construction} & Asymmetric encryption & Symmetric encryption 
 %   & Public key encryption 
 %   & \Sigma-protocol zero-knowledge 
%    & Semantic security \\
 %   \hline 
%    \textit{Main Security Theorem} 
 %   & Reduces \emph{one-time}-CPA security of ElGamal to DDH problem 
 %   & Indist (IND-CPA) by bounding $\mathcal{A}$'s advantage  
 %   & Indist by reducing $\mathcal{A}$'s advantage to the security of underlying primitives. KEM and DEM are secure against chosen ciphertext (IND-CCA). 
 %   & Indist in the context of zero-knowledge proof. Convert the class of \Sigma protocol into a commitment scheme  
 %   & Reduces the security of \ra to the security of digital signatures \\ 
 %   \hline
 % \end{tabular}
 % \caption{IND formalization examples in \ssprove}\label{tab:ind-lib}
%\end{table}
%\end{minipage}
%In this paper, we formally specified digital signatures as the foundation of remote attestation in the theorem prover \coq.
%To the best of our knowledge, we are the first to do so in the context of game-based proofs that rely on
%the security notion of indistinguishability.
%
During our formal development, we noticed a difference between the traditional definitions in the textbook~\cite{joy}
on indistinguishable signatures and SSProve, a framework 
that followed such a textbook to implement formal indistinguishability reasoning. 
%
There exist two perspectives: one of the textbook authors, 
i.e., leading cryptographers, and one of the authors of
\ssprove, i.e., leading experts in the design of formal
reasoning tools and programming languages.
%
We present the views and then discuss their implications.
%

\subsection{Indistinguishable Signatures in Textbooks}
%
The textbook definitions of indistinguishability for digital signatures lack precision. 
%
The definition of the \emph{game pair} for digital signatures
in Figure~\ref{fig:problem:ind} of Section~\ref{sec:TheoryFound}
follows the textbook ``The Joy of Cryptography'' (\joc)~\cite{joy} and
``Companion to Cryptographic Primitives, Protocols and Proofs'' (\companion)~\cite{companion}.
%
\joc defines the advantage of an adversary exactly as \ssprove does, 
and the \companion follows a comparable approach. 
%
%\begin{minted}[escapeinside=@@]{Coq}
%Definition Adv A G@$_1$@ G@$_2$@ := @$|$@ A @$\circ$@ G@$_1$@ - A @$\circ$@ G@$_2$@ @$|$@.
%\end{minted}
%
%The definition in the \companion is similar.
%
\joc acknowledges that packages are essentially an
abstraction for libraries, as in languages such as Java, 
which may have more than one procedure (see Definition~2.3).
%
The \companion explicitly refers to these procedures as oracles (see Section~2.3).
%
However, neither \joc nor \companion formally defines what it means for a package 
with multiple procedures to be indistinguishable, leading to a gap in the literature. 
%
To address this, we propose that indistinguishability in such settings should be 
defined based on the behavior of the adversary interacting with a real and an ideal package. 
%
Specifically, a signature scheme's real and ideal packages consist of three procedures: \egetpk, \esign, and \eversig. 
%
The adversary interacts with these procedures as a black-box access point within the library—yet existing 
literature abstracts over this interaction without providing formal proof of indistinguishability. 
%
Establishing such a definition ensures a rigorous foundation for reasoning about multi-procedure cryptographic games. 

\subsection{Indistinguishable Signatures in \ssprove}
\begin{figure}
	\centering
  \begin{subfigure}[0]{\columnwidth}
    \centering
    \input{tikz/versig-game}
    \caption{Game}
    \label{fig:versig:game}
  \end{subfigure}
\\[0.3cm]
	\begin{subfigure}[0]{0.7\columnwidth}
    \centering
%    \input{tikz/sig-prop}
		\begin{minted}[fontsize=\footnotesize,escapeinside=@@,autogobble]{coq}
      @$\forall$@ pk m S s, VerSig pk s m = ((m, s) @$\in$@ S)
		\end{minted}

    \caption{Property}
    \label{fig:versig:prop}
  \end{subfigure}

	\caption{
    %
    The game for the \eversig procedure requires a
    property that cannot be instantiated.
    %
  }
	\label{fig:versig}
\end{figure}

%
The \ssprove authors followed the \joc textbook, adapting its indistinguishability
definifions for implementation~\cite{ssprove}\footnote{\url{https://github.com/SSProve/ssprove/tree/main/theories/Crypt/examples}}.
%
%and implemented various examples from the book~\cite{ssprove2021}\footnote{\url{https://github.com/SSProve/ssprove/tree/main/theories/Crypt/examples}}.
%
Of course, for the implementation of \ssprove, the authors
had to be specific about what it means for a library to be a 
indistinguishable.
%
They chose the most natural definition:
two libraries are indistinguishable when each of their
procedures are indistinguishable.
%
Hence, an adversary package's advantage is essentially
accumulating the advantages for the individual procedures.
%
However, that has severe implications for the definition
of indistinguishability for digital signatures.
%

%
Recall the definition of \eversig from the game in Figure~\ref{fig:sigprim:packages}, 
now shown in Figure~\ref{fig:versig:game}, with a better view for readers. 
%
The indistinguishability proof requires the property in Figure~\ref{fig:versig:prop} to hold.
%According to the indistinguishability proof, the property must eventually be in Figure~\ref{fig:versig:prop}.
%
However, this property can never be established—only 
the right-hand side of the property talks about
the set of already generated signatures \mintinline{Coq}{S}.
%
The property misses the assumption that
the signature ($s$) was generated by
a call to \esign.
%
Consequently, existing textbook definitions cannot prove the 
indistinguishability of signature primitives in isolation. 
%As a result, the definition as presented in the textbooks cannot be proven.
%That is, the primitives of a signature scheme cannot be proven individually. \todo{Jannik: unclear sentence (from the property misses..)}
%Only the protocol, as stated in Figure~\ref{fig:problem:eu-ind} of Section~\ref{sec:TheoryFound} can be proven indistinguishable.
%
Instead, only complete protocols—such as the one in Figure~\ref{fig:problem:eu-ind} 
of Section~\ref{sec:TheoryFound}—can be rigorously proven indistinguishable.

\subsection{Discussion}
%
Two options exist to resolve this inconsistency.
%
On the one hand, it may be that the cryptographers
intuitively meant that signatures can only ever be
generated by \esign.
%
If that is the case, frameworks such as \ssprove
would have to change and add such an assumption
into the context for the proof of \eversig.
%
Indeed, the Diffie-Hellman Key Exchange and ElGamal 
definition has the protocol stated explicitly
(see Chapters~14 and 15).
%
On the other hand, at least for signature schemes,
the according proof would be very much the same
as stated in our protocol definition.
%
As such, adjusting them according to textbook sections might be justified.
%
We do not take a side at this point and leave it
as a discussion to the community.
%

However, this discussion of discrepancy is an important issue for future research. 
%
We all know that traditional cryptographic textbooks generally present abstract definitions 
and omit some implementation steps for simplification. 
%
However, these definitions are becoming very difficult to build our 
intuition upon, and they deviate from the rigorous demands 
of the proof framework, which requires detailed and precise formalization of these definitions. 
%
Furthermore, our formal development also shows the proof phase related to indistinguishability that, 
to our knowledge, has not been previously addressed by SSProve experts in their existing examples. 
%
This highlights a gap, and we try our best to bridge it through our proof engineering. 
%

During our formal development, we successfully proved the 
indistinguishability of \real and \ideal games for most routines. 
%
However, one invariant \texttt{sig\_inv} fails in the initial state. 
%
This structural mismatch appears because the invariant assumes an operational 
state with initialized keys and mappings for signed operations. 
%
Nevertheless, the empty state lacks these structures, which leads to a 
semantic gap that prevents the invariant from being proven. 
%
This structural mismatch does not affect our security guarantees.
%
In practical systems, when the protocol starts, the controlled initialization ensures the invariant holds, 
which makes the empty state irrelevant to operational security. 
%
%
%\begin{table}%[p] \centering
 % \begin{tabular}{ | p{0.58in} | p{1.4in} | p{1.2in} |}
 %   \hline
 %   \textbf{Aspects} & \textbf{Our proof development} & \textbf{\ssprove examples} \\[0.5ex] 
 %   \hline
 %    \textit{Packages} & Tend to focus on multi-purpose packages 
 %                       to integrate multi procedures to attain 
 %                       complex functionalities.
 %                      & Tend to focus on single-purpose packages, 
 %                      dedicated to specific cryptographic primitives. \\
 %                      %\hline
 %     \textit{Challenges} & Specific case (\ra) and introduced protocol-specific 
  %                          invariants which is difficult with reasonings.
 %                         & Proofs are based on game-hopping with simpler transitions. \\
 %     \textit{Focus}   &  Manual and customized lemmas for libraries, 
 %                         the indistinguishability spans across multiple 
 %                        exported procedures and adversary's cases.
 %                      & Generic cryptographic primitives and limited 
%                         to reason about isolated procedures calls. \\              
%     \hline
%  \end{tabular}
%\end{table}



%


%\todo{go to elgamal, see if they do the indistinguishability: would they have the same problem as we (protcol thing / definition insufficien)}
%\todo{look at ref. 15, see if they have encountered the same protocol-primitive problems (same as above in elgamal)}




==> src/signatures.tex <==
\section{A Formal Specification for Digital Signatures}\label{sec:sig}
%
%
We formally specify and verify the security of digital signature schemes using the \ssprove framework.
%
This section introduces the modular specification of signatures, 
the abstraction of key generation, signing, and verification, and the construction of real and ideal signature protocols. 
%
We then prove their perfect indistinguishability. 
This section serves as a foundation for securing \ra in Section~\ref{sec:vra}.
%
%
\subsection{Overview and Intuition}
Note that our formal development for both digital signature and \ra is structured around two components: 
the composition of modular packages and the formal proof of their security properties.
%
Figure~\ref{fig:overview} illustrates the modular composition of the digital signature 
and \ra specification. 
%
Real-world protocols are represented in grey, 
while idealized protocols are shown in yellow. 
%
Each component is specified as an \ssprove package.
%
The \pkeygen handles key generation, SigPrim for primitives, and SigProt composes these into protocols, 
and similar names such as AttPrim and AttProt apply for \ra. 
%
The specification is parameterized by a signature scheme $\Sigma$ consisting of a key generation algorithm $\Sigma$.\pkeygen, 
a signing function $\Sigma$\icoq{.Sign}, and a verification function $\Sigma$.\icoq{VerSig}, 
all defined abstractly over finite types. 
%
The specification centers around the \pkeygen package, which abstracts the key generation process. 
%
We aim to model signatures in a way that abstracts over concrete implementations (like RSA or ECDSA) 
while capturing essential cryptographic properties such as strong existential unforgeability (sEUF-CMA). 
%
An example instantiation for RSA signatures is provided in Appendix~\ref{sec:rsa}.
%
\begin{figure*}
	\centering
	\input{tikz/overview}
	\caption{
  %
  Our formal specification of remote attestation is based on digital signatures.
  %
  The security reasoning is based on the concept of indistinguishability
  for a game pair \real, which represents the actual code,
  and \ideal, which represents the model, i.e., the semantics
  of the real code
  in the context of indistinguishability proofs.}\label{fig:overview}
\end{figure*}
%
%
The proof development demonstrates that the composition of these packages suffices to establish 
strong security guarantees for the digital signature scheme. 
%
We formally prove that strong existential unforgeability under chosen message attacks (sEUF-CMA) 
implies indistinguishability between the real and ideal signature protocols. 
%
The core intuition behind the proof of indistinguishability is rooted in the sEUF-CMA property. 
%
If an adversary cannot forge a signature on any new message, then all accepted 
signatures must have been generated via the signing interface. In this case, 
the behavior of the real and ideal protocols is indistinguishable from the adversary’s point of view.
%
If an adversary could distinguish between the two protocols, 
it must have found a message for which the real protocol accepts a signature while the ideal protocol rejects it. 
%
This would require forging a signature on a message not previously signed—a direct contradiction to strong unforgeability.
%
Conversely, if a signature scheme is forgeable, 
the adversary can trivially distinguish the real and ideal games by submitting the forged signature. 
%
Hence, indistinguishability characterizes unforgeability and vice versa.
%

We formalize this reasoning and prove the following results. 
%
Theorem~\ref{theo:indist-signature} establishes Perfect Indistinguishability between the real and ideal digital signature protocols. 
%
Theorem~\ref{theo:redprot} establishes a reduction theorem showing that the security of remote attestation is at least as strong as the security of the underlying digital signatures. 
%
Theorem~\ref{theo:indist-ra} combines the two results to conclude that remote attestation satisfies strong existential unforgeability.
%
%

\begin{wrapfigure}{r}{0.32\textwidth}
  \centering
  \input{tikz/keygen-pkg}
  \caption{Package}
  \label{fig:keygen:package}
\end{wrapfigure}
\vspace{-1.2em}
%
\subsection{Key Generation}
Following the definition of signatures, we formalize key generation.
%We start by formalizing key pair generation.
The \pkeygen package,
abstracts the key generation process over arbitrary finite types for the secret key (\lseckey) and public key (\lpubkey). 
%
The package is parameterized by a key generation algorithm $\Sigma$.\pkeygen, which samples key pairs from a distribution.
%
Unlike the classical approach, which often models key generation as a pure function, 
we model $\Sigma$.\pkeygen as a probabilistic sampling procedure. 
%
This design choice ensures compatibility with the security game framework, 
where packages must use explicit probabilistic operations and cannot rely on external sources of randomness.
%
Therefore, the \pkeygen package exports the procedure %\ekeygen. 
\ekgen, 
which samples a key pair using $\Sigma$.\pkeygen, stores it in the local state, and returns the result. 
%
The signing and verification procedures later retrieve this stored key material. 
%
Crucially, $\Sigma$.\pkeygen must be polymorphic in this state, ensuring that the sampling 
process is side-effect-free for the external state of the composed packages. 
%
This technique enables the clean composition of \pkeygen with the signature primitives while preserving soundness guarantees.

%
Having defined key generation, we now formalize the signing and verification components.
%
%
%%%%%% This figure needs to be sorted
%\begin{wrapfigure}{r}{0.4\textwidth}
 % \centering
  %\input{tikz/prot-pkg}
  %\caption{The protocol package for digitial signatures}
  %\label{fig:pprot}
%\end{wrapfigure}
%
\subsection{Signature Primitives}
We now define the signing and verification primitives abstractly over Message and Signature types. 
%
The signing function $\Sigma$\icoq{.Sign} takes a secret key and a message and outputs a signature. 
%
The verification function $\Sigma$.\icoq{VerSig} takes a public key, a message, 
and a signature and outputs a Boolean indicating whether the signature is valid. 
%
Both operations are deterministic and do not modify the package state.
%

The following hypothesis captures the functional correctness of the signature scheme:
%
\begin{hypothesis}[functional correctness]
\[   \forall m sk pk,
  ((sk, pk) \leftarrow \Sigma.\text{\pkeygen}) \rightarrow \\
  \Sigma.\text{\icoq{VerSig}} pk (\Sigma\text{\icoq{.Sign}} sk m) m == true.
\] 
\end{hypothesis}
%
%
\begin{figure}
  \centering
  \input{tikz/sig-real-vs-ideal}
  \caption{The \real and \ideal Signature Primitives packages.}
  \label{fig:sigprim:packages}
\end{figure}
%
That is, for any key pair generated 
by $\Sigma$.\pkeygen and any message $m$,
signing, and then verifying should succeed.
%
%

We implement two versions of the signature primitive packages (Figure~\ref{fig:sigprim:packages}). 
%
The real version directly implements the signing and verification operations, 
invoking $\Sigma$\icoq{.Sign} and $\Sigma$.\icoq{VerSig} respectively. 
%
The ideal version tracks an internal set \icoq{S} of signed messages and 
accepts a signature during verification only if it 
corresponds to a message previously signed through the signing interface.
%
Both packages rely on the \egetpk procedure from \pkeygen to retrieve the \icoq{pk}. 
%

With the primitives in place, we now describe the composition of the real and ideal protocols 
and the security proof that establishes their indistinguishability.
%
%
\subsection{Indistinguishability Proof}
We construct the real and ideal digital signature protocols to formalize the 
security property by composing the primitives with the key generation package. 
%
The composed protocols are defined as follows:
%
\begin{definition}[\psigprot$_{\text{\real}}$]\label{def:sigprotR}
  \( \{\)package \psigprot \circledcirc \, \psigprim$_{\text{\real}}$ \circ \, \pkeygen\( \}\).
\end{definition}
%
\begin{definition}[\psigprot$_{\text{\ideal}}$]\label{def:sigprotI} 
  \( \{\)package \psigprot \circledcirc \, \psigprim$_{\text{\ideal}}$ \circ \, \pkeygen\( \}\).
\end{definition}
%
The wrapper package \psigprot relabels the procedures of the 
signature primitives to provide a unified interface (special notation $\circledcirc$). 
%
Specifically, it renames the \esign operation to \icoq{challenge} and 
the verification operation \eversig to \icoq{verify}%
\footnote{
%
In \ssprove, this is not necessary because procedure names map
to a particular natural number.
%
Mapping different procedure names to the same natural numbers
establishes the link without an auxiliary package for renaming
procedures.
%
}. 
%
This relabeling ensures that the composed packages match the 
interface and are comparable to the security proof.
%

We then establish our main result:
%
\begin{theorem}[Perfect Indistinguishability of Digital Signatures]\label{theo:indist-signature}
  %
  For every adversary \A, the advantage to distinguish the packages
  \psigprot$_{\text{\real}}$ and \psigprot$_{\text{\ideal}}$ is $0$:
  %
  
  \qquad \qquad \qquad \qquad \psigprot$_{\text{\real}}$ \pindist \psigprot$_{\text{\ideal}}$.
\end{theorem} 
%
\begin{proof}
  The proof proceeds by establishing an invariant \icoq{heap_ignore} (Figure~\ref{fig:ind:proof})
  that the heap states of the real and ideal packages are identical 
  up to an irrelevant location $\mathcal{SIG}$.
  %
  As the protocols evolve, this invariant is preserved through every execution step, ensuring that signing 
  and verification operations behave identically from the adversary’s perspective.
  %
  The critical point in the proof is to show that any observable difference 
  between the real and ideal games would require a signature to verify 
  correctly in the real protocol without having been produced by 
  the signing interface in the ideal protocol. 
  %
  However, this is ruled out by the signature scheme's functional correctness property (Definition\ref{def:sig:correct}). 
  %
  Thus, any adversary interacting with the two packages will 
  observe identical behavior, and no distinguishing advantage is possible.
\end{proof}
%
As discussed in the following sections, the indistinguishability result forms the foundation 
for analyzing higher-level cryptographic protocols, including \ra.
%
\begin{figure}
  \begin{minipage}{0.25\columnwidth}
  \begin{minted}[escapeinside=@@,fontsize=\scriptsize,autogobble]{Coq}
  @$\vdash$@
  { @$\lambda$@ (s@$_1$@, s@$_2$@),
    let inv := heap_ignore @$\{\mathcal{SIG}\}$@ in
    let h   := inv @$\rtimes$@ rm_rhs @$\mathcal{SIG}$@ S in
    let h'  := set_rhs @$\mathcal{SIG}$@ (S @$\cup$@ @$\{$@(@$\Sigma$@.Sign sk m, m)@$\}$@ h in
    let h'' := h' @$\rtimes$@ rm_rhs @$\mathcal{SIG}$@ S' in
    h'' (s@$_1$@, s@$_2$@)) }
  ret (pk, @$\Sigma$@.Sign sk m, @$\Sigma$@.VerSig pk (@$\Sigma$@.Sign sk m) m)
  @$\approx$@
  ret (pk, @$\Sigma$@.Sign sk m, (@$\Sigma$@.Sign sk m, m) @$\in$@ S')
  { @$\lambda$@ (s@$_1$@,r@$_1$@)
      (s@$_2$@,r@$_2$@), r@$_1$@ = r@$_2$@ @$\land$@ heap_ignore @$\{\mathcal{SIG}\}$@ (s@$_1$@, s@$_2$@) }
  \end{minted}
  \end{minipage}
  \caption{
    %
    Theorem~\ref{theo:indist-signature} %\icoq{SigProt_}$\mathcal{G}_{\text{\pindist}}^{\Sigma}$ 
    reduces to functional correctness. 
    %
  }\label{fig:ind:proof}
  \end{figure}
  %
  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\out{ %%%%%%%%%%%%%%%%%%%%%% COMMENT out
In this section, we present our formal specification of digital
signatures and verify that it is secure against forgery. 
%
First, we present an overview of our specifications and fix their notations.
%
Afterwards, we specify the package for key generation.
%and state its assumptions for concrete implementations such as RSA. 
%
Then, we followed the specifications for digital signatures. 
%
First, we define the packages and then provide details for proof of 
game-based indistinguishability (perfect).
%

\subsection{Overview and Notations}
%
Our development has two parts: the composition of the packages
and the proof development to establish the security properties.
%

\subsubsection{Package Composition}

\begin{figure*}
	\centering
	\input{tikz/overview}
	\caption{
  %
  Our formal specification of remote attestation is based on digital signatures.
  %
  The security reasoning is based on the concept of indistinguishability
  for a game pair \real, which represents the actual code,
  and \ideal, which represents the model, i.e., the semantics
  of the real code
  in the context of indistinguishability proofs.}\label{fig:overview}
\end{figure*}


\begin{figure}
  \centering
  \input{tikz/prot-pkg}
  \caption{The protocol package for digitial signatures.}
  \label{fig:pprot}
\end{figure}
%
Figure~\ref{fig:overview} visualizes our specification using SSP-style
visualization for package composition.
%
In the figure, we accordingly highlight \real (shaded in grey) and 
\ideal (shaded in yellow) packages.
%
Our specification builds upon a key generation package \pkeygen that
establishes the probabilistic foundation.
%
The package \pkeygen abstracts over a concrete foundation to allow
for various instantiations such as RSA and ECDSA.
%
A full specification for the instantiation with RSA is in Appendix~\ref{sec:rsa}
with the details in the proof development.
%
The package \pkeygen exports a \ekeygen procedure for the packages that
define the \real and \ideal signature
primitives.
%
%Figure~\ref{fig:problem:eu-ind} shows that the composition of \prot \sa{SigProt?} with 
%packages \real and \ideal for signature
%primitves instantiates the protocol for digitial signatures.
%
%The protocol remains unchanged for remote attestation such that
%we can compose \pprot similarly with the \real and \ideal packages 
%for the remote attestation primitives.
%

\subsubsection{Proof Development}
%
Our proof development shows that our structured approach proves 
the security of signatures by establishing an equivalence between 
sEUF-CMA and indistinguishability-based security. 
%
The main idea is that if a signature scheme is secure with strong unforgeability, 
then the probability of forging a valid signature for the previously signed message is negligible. 
%
The signature verification in $\mathcal{G}_{\real}^{\Sigma}$ returns true with a valid message-signature pair. 
%
By the definition of strong unforgeability assumption, the $\mathcal{G}_{\ideal}^{\Sigma}$ must also return true, 
as any valid signature must have been generated by singing primitive. 
%
This ensures that the real and ideal signature verification processes remain indistinguishable. 
%
Contrariwise, if the real and ideal signature packages are 
indistinguishable, it implies that the ideal one must also 
accept any valid message-signature pair accepted by the real package. 
%
If an adversary could forge a valid signature, the real package would return \emph{true}, 
while the ideal package would return \emph{false}. 
%
By ensuring that the adversary can not distinguish these two cases, 
we naturally guarantee that forging a new signature is infeasible. 
%
This reasoning extends to both fresh and previously signed messages, which leads 
to the judgment that indistinguishability implies sEUF-CMA. 
%

Our proof construction establishes indistinguishability, i.e.,
strong existential unforgeability, for digital signatures based on
the protocol packages (Theorem~\ref{theo:indist-signature}). 
%
Theorem~\ref{theo:redprot} is a reduction theorem and states that
the security of remote attestation is smaller or equal to the
security of digital signatures.
%
Theorem~\ref{theo:indist-ra} then uses Theorem~\ref{theo:indist-signature}
and Theorem~\ref{theo:redprot} to verify strong existential
unforgeability of remote attestation.
%

\subsection{Key Generation}

\begin{figure}
	\centering
    \begin{subfigure}[b]{\columnwidth}
    \centering
       \begin{minted}[fontsize=\footnotesize,escapeinside=@@,autogobble]{coq}
Parameters SecKey PubKey : finType.
Parameter  @$\Sigma$.@KeyGen : @$\forall$@ s, code s (PubKey × SecKey).
		  	\end{minted}
      \caption{Parameters.}
	    \label{fig:keygen:params}
    \end{subfigure}
\\[0.3cm]
  \begin{subfigure}[b]{\columnwidth}
    \centering
    \input{tikz/keygen-pkg}
    \caption{Package.}
    \label{fig:keygen:package}
  \end{subfigure}
  \caption{
    %
    The \pkeygen package and its parameters.
    %
  }
  \label{fig:keygen}
\end{figure}

%
Following the (textbook) definitions from Section~\ref{sec:TheoryFound},
we define the package \pkeygen in Figure~\ref{fig:keygen}.
%
We leave the definition of the secret key (\lseckey)
and the public key (\lpubkey) abstract as parameters
and just require them to be of a finite type.
%
Similarly, we parameterize the package with an algorithm
$\Sigma$.\pkeygen that implements the final key generation.
%
We do not import this algorithm because otherwise, we cannot play
the security game: game packages cannot have imports.
%
The algorithm $\Sigma$.\pkeygen nevertheless emits monadic code
because it needs to sample the keys from a distribution.
%
This differs from the textbook definition, which states that the $\Sigma$.KeyGen
is a pure function.
%
The $\Sigma$.\pkeygen is polymorph in the state \icoq{s}, i.e.,
it has no side-effects to the state other than for sampling.
%
The \egetpk procedure stores the generated secret and public
keys into its state and returns them both.
%
We are now ready to specify digital signatures.
%
We start with defining the primitives, and
afterwards, we compose the protocol games to prove perfect indistinguishability, 
i.e., strong existential unforgeability for digital signatures.
%
\subsection{Primitives}

\begin{figure}
	\centering
   \begin{subfigure}[b]{\columnwidth}
    \centering
        \begin{minted}[fontsize=\footnotesize,escapeinside=@@,autogobble]{coq}
Parameters Message Signature : finType.
Parameter  @$\Sigma$@.Sign : SecKey -> Message -> Signature.
Parameter  @$\Sigma$@.VerSig :
  PubKey -> Signature -> Message -> bool.
	\end{minted}
    \caption{Parameters}
    \label{fig:sigprim:params}
  \end{subfigure}
\\[0.3cm]
   \begin{subfigure}[b]{\columnwidth}
    \centering
        \begin{minted}[fontsize=\footnotesize,escapeinside=@@,autogobble]{coq}
Hypothesis sig_correct :
  @$\forall$@ m sk pk,
    ((sk,pk) <- @$\Sigma$@.KeyGen) ->
    @$\Sigma$@.VerSig pk (@$\Sigma$@.Sign sk m) m == true.
	\end{minted}
    \caption{Functional Correctness}
    \label{fig:sigprim:hypo}
  \end{subfigure}
\\[0.3cm]
\begin{subfigure}[b]{\columnwidth}
    \centering
    \input{tikz/sig-real-vs-ideal}
    \caption{Packages}
    \label{fig:sigprim:packages}
  \end{subfigure}
	\caption{
    %
    The \real and \ideal Signature Primitives packages
    and their parameters and hyptohesis.
    %
    }
	\label{fig:sigprim}
\end{figure}

%
Figure~\ref{fig:sigprim} defines the abstractions and then
specifies the primitives for our digital signatures.
%

%
In line with the (textbook) definition presented in
Figure~\ref{fig:problem:ind}, our implementation of
the signature primitives abstracts over a concrete
signature scheme.
%
In Figure~\ref{fig:sigprim:params}, we abstract over concrete
implementations for messages and signatures.
%
The abstractions for signing a message and verifying a signature
complete Definition~\ref{def:sig:scheme} of a signature scheme $\Sigma$.
%
Note that both $\Sigma$\icoq{.Sign} and $\Sigma$.\icoq{VerSig}
are pure functions because they neither sample nor access any state.
%
Functional correctness (Definition~\ref{def:sig:correct}) is then
a hypothesis of our primitives for digital signatures (Figure~\ref{fig:sigprim:hypo}).
%
We specify the \real and \ideal packages for the primitives
of our digital signatures in Figure~\ref{fig:sigprim:packages}.
%
Our specification pays attention to accessing and updating
the state, e.g., for the set \icoq{S} of observed signatures in the
\ideal package.
%
Both packages import \ekeygen to obtain the
public key \icoq{pk}.
%
Note again that \ekeygen stores the generated keys \icoq{sk}
and \icoq{pk} into its state.
%
Respectively, the state of \pkeygen needs to be a
subset of the state of each package such that \esign and
\eversig can access the keys.
%
Apart from these implementation details,
both package definitions follow the (textbook)
specification from Figure~\ref{fig:problem:ind}.
%
\subsection{Indistinguishability}

\begin{figure}
    \begin{minted}[fontsize=\footnotesize,escapeinside=&&,autogobble]{coq}
Definition SigProt&$_{\text{\real}}$& :=
  {package SigProt &$\circledcirc$& SigPrim&$_{\text{\real}}$& &$\circ$& KeyGen}.

Definition SigProt&$_{\text{\ideal}}$& :=
  {package SigProt &$\circledcirc$& SigPrim&$_{\text{\ideal}}$& &$\circ$& KeyGen}.
    \end{minted}
   \caption{Protocol games for digital signatures.}
   \label{fig:sigprot}
\end{figure}

%We prove security against forgery for our digital signaturesbased on the generic protocol \pprot.
%In order to establish the game for this proof, we need a \real and \ideal protocol package.
%We construct both packages via package composition.
%
To prove the security against forgery for our digital signatures, 
we establish a \emph{game pair} for this security proof. 
%
We construct a \real and \ideal protocol package, as shown in Figure~\ref{fig:sigprot}. 
%
The \real protocol package
\psigprot$_{\text{\real}}$ is a composition of packages
Sig\prot, \psigprim$_{\text{\real}}$ and \pkeygen. 
%\pkeygen, \psigprim$_{\text{\real}}$ and \pprot.
%
The respective \ideal package
\psigprot$_{\text{\ideal}}$ is a composition of packages
Sig\prot, \psigprim$_{\text{\ideal}}$ and \pkeygen.
%pkeygen, \psigprim$_{\text{\ideal}}$ and \pprot.
%
We use the special notation $\circledcirc$ to denote a composition
up to renaming procedures \esign to \icoq{challenge} and
\eversig to \icoq{verify}%
\footnote{
%
In \ssprove , this is not necessary because procedure names map
to a particular natural number.
%
Mapping different procedure names to the same natural numbers
establishes the link without an auxilary package for renaming
procedures.
%
}.
%
The game that we play, and respectively, the theorem that we prove,
establishes perfect indistinguishability between the \real and 
the \ideal protocol package (Figure~\ref{fig:sigprim:packages}).

%
\begin{theorem}[%\icoq{SigProt_}$\mathcal{G}_{\text{\pindist}}^{\Sigma}$: 
  Perfect Indistinguishability of Digital Signatures]\label{theo:indist-signature}
  %
  For every attacker \A, the advantage to distinguish the packages
  \psigprot$_{\text{\real}}$ and \psigprot$_{\text{\ideal}}$ is $0$:
  %
  \begin{center}
    \begin{minipage}{0.5\columnwidth}
    \begin{minted}[fontsize=\footnotesize,escapeinside=&&,autogobble]{coq}
SigProt&$_{\text{\real}}$& &$\pindist$& SigProt&$_{\text{\ideal}}$&.
    \end{minted}
    \end{minipage}
    \end{center}
\end{theorem} 

%
\begin{figure}
\begin{center}
\begin{minipage}{0.9\columnwidth}
\begin{minted}[escapeinside=@@,fontsize=\footnotesize,autogobble,linenos]{Coq}
@$\vdash$@
{ @$\lambda$@ (s@$_1$@, s@$_2$@),
  let inv := heap_ignore @$\{\mathcal{SIG}\}$@ in
  let h   := inv @$\rtimes$@ rm_rhs @$\mathcal{SIG}$@ S in
  let h'  := set_rhs @$\mathcal{SIG}$@ (S @$\cup$@ @$\{$@(@$\Sigma$@.Sign sk m, m)@$\}$@ h in
  let h'' := h' @$\rtimes$@ rm_rhs @$\mathcal{SIG}$@ S' in
  h'' (s@$_1$@, s@$_2$@)) }
ret (pk, @$\Sigma$@.Sign sk m, @$\Sigma$@.VerSig pk (@$\Sigma$@.Sign sk m) m)
@$\approx$@
ret (pk, @$\Sigma$@.Sign sk m, (@$\Sigma$@.Sign sk m, m) @$\in$@ S')
{ @$\lambda$@ (s@$_1$@,r@$_1$@)
    (s@$_2$@,r@$_2$@), r@$_1$@ = r@$_2$@ @$\land$@ heap_ignore @$\{\mathcal{SIG}\}$@ (s@$_1$@, s@$_2$@) }
\end{minted}
\end{minipage}
\end{center}

\caption{
  %
  The final step in the proof of the Theorem \icoq{SigProt_}$\mathcal{G}_{\text{\pindist}}^{\Sigma}$ reduces it to \icoq{sig_correct}.
  %
}
\label{fig:ind:proof}
\end{figure}
%
%
\begin{IEEEproof}
%[Proof of \icoq{SigProt_}$\mathcal{G}_{\text{\pindist}}^{\Sigma}$]
The according proof (game) is a straight forward application of
\ssprove tactics that reduce the goal to the judgement in Figure~\ref{fig:ind:proof}.
%
We use the \icoq{heap_ignore} invariant that is already defined in
\ssprove to state that
\icoq{s}$_1$, the state of the \real package, and
\icoq{s}$_2$, the state of the \ideal package are equal up to
the $\mathcal{SIG}$ location.
%
The proof process extends this invariant in the precondition
with a trace of reads from state into local variables and
updates to state (Lines~4--6).
%
The commands for the \real (left) and \ideal (right) commands
are equal up to the third element of the returned triple.
%
Clearly, the trace contains the evidence (Line~5) that the
signature--message pair really is in \icoq{S'} (Line~10).
%
This allows us to reduce the indistinguishability to the equality
%
\begin{minted}[escapeinside=@@,autogobble]{Coq}
@$\Sigma$@.VerSig pk (@$\Sigma$@.Sign sk m) m = true
\end{minted}
%
which is the functional correctness Hypothesis \icoq{sig_correct}
of the signature scheme $\Sigma$.
%
\end{IEEEproof}

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


==> src/ssprove.tex <==
\section{Foundationally Proving Indistinguishability using SSProve}
\label{sec:ssprove}
\sa{This section needs to go away but we need the below command lines in sec2.}




%
\ssprove is a \coq library that implements the State
Separation Proof (\ssp) methodology to provide a framework
for cryptographic proofs~\cite{ssp}.
%
This section gives a brief introduction and defines the notiation
that we use in the next sections for our formalization.\footnote{
Readers familiar with SSP can safely skip this section.}
%
First, we introduce packages and the syntactical constructions
to implement them.
%
Afterwards, we describe game-based security proofs as the
foundation to reasoning about security semantically.
%

\paragraph{Packages}

%
A packages in \ssprove defines a set of procedures that
operate on a common state.
%
We present a simple package in Figure~\ref{fig:package}.
%
A package \emph{imports} procedures, i.e., procedure types,
and \emph{exports} own procedures.
%
Package \p defines and exports procedure \z.
%
The definition of \z depends on imported procedure types
\x and \y.
%
\ssp defines and \ssprove implements sequential composition
$\circ$ for packages.
%
For example, $\oo \circ \p$ requires \oo
to define procedures \x and \y.
%

%
For the definition of a procedure, \ssprove provides
a language that is based on the notion of a state monad \mintinline{Coq}{code}
to account for operations on the package state
and sampling from distributions~\cite{10.1145/143165.143169}.
%
The \cget and \cput commands allow monadic read and write
access to state locations.
%
To keep the listings concise, we abstract over the
locations and denote \mintinline{Coq}{@}$\mathcal{S}$ to denote
the memory location for \mintinline{Coq}{@}$\mathcal{S}$.
%
Other monadic operations are \cassert statements
and sampling values (\csample) from a probability
distribution over finite spaces\footnote{\mintinline{Coq}{n <$} $\mathbb{N}_6$ is
notation for \mintinline{Coq}{n <- sample} $\mathbb{N}_6$.}.
%
\ssprove allows to embedded \coq expressions such as
\mintinline{Coq}{z + n} into the code of a procedure.
%
Values may enter into the \mintinline{Coq}{code} monad
via the usual \cret command.
%
Throughout the paper, we mark all commands with a \texttt{\#}.
%
All imports and exports are monadic procedures and
part of the composition requires to match up the
states of the composed packages.
%
For the imports and export of the example package \p
in Figure~\ref{fig:package}, we omitted this detail.
%

%
\paragraph{Game-based Proofs}
%
Indistinuishability proofs in \ssprove are game-based.
%
A \emph{game} is simply a packages with no imports.
%
A \emph{game pair} is then a pair of packages with the same
exports.
%
An industinuishability statement about two games
\mintinline{Coq}{G}$_1$ and \mintinline{Coq}{G}$_2$
reasons about the advantage of an attacker.
%
An \emph{attacker} is a package that imports all
exports from game packages.
%
That is, the adavantage of an attacker \mintinline{Coq}{A}
is simply
%
\begin{minted}[escapeinside=@@]{Coq}
Definition Adv A G@$_1$@ G@$_2$@ := @$|$@ A @$\circ$@ G@$_1$@ - A @$\circ$@ G@$_2$@ @$|$@.
\end{minted}
%
\se{
  %
  Indeed what does that actually mean when a package composition
  produces a real number.
  %
  At this point, this does not matter.
  %
  We need detail this point in the implications section.
  %
}
%
For the upcoming section, it suffices to understand that
indistinguishability \mintinline{Coq}{G}$_1 \indist$ \mintinline{Coq}{G}$_2$ means
%
\begin{minted}[escapeinside=@@]{Coq}
Adv A G@$_1$@ G@$_2$@ = 0.
\end{minted}
%
In Section~\ref{sec:imply}, we get back to the interesting
question of what it actually means for a package to produce
a real number.
%
Proof-reasing follows \textit{probabilistic relational Hoare logic} (pRHL)~\cite{barthe2009formal}.
%
Judgements in this logic are hoare triples
%
%
%@$\vDash\big\{(s_1,s_2).\phi\big\}\;c_1\thicksim c_2\;\big\{((s_1',r_1),(s_2',r_2)),\psi\big\}$$
\begin{minted}[escapeinside=@@,fontsize=\footnotesize,autogobble]{Coq}
  @$\vdash$@ { @$\lambda$@ (s@$_1$@,s@$_2$@), @$\phi$@ } c@$_1$@ @$\approx$@ c@$_2$@ { @$\lambda$@ ((s@$_1$@',r@$_1$@),(s@$_2$@',r@$_2$@)), @$\psi$@ }
\end{minted}
%
where the pre-condition $\phi$ is a proposition about initial states
\mintinline{Coq}{s}$_1$, \mintinline{Coq}{s}$_2$
and the post-condition $\psi$ is a proposition about the final states
\mintinline{Coq}{s}$_1'$, \mintinline{Coq}{s}$_2'$
and the results
\mintinline{Coq}{r}$_1$, \mintinline{Coq}{r}$_2$
produced by the commands
\mintinline{Coq}{c}$_1$, \mintinline{Coq}{c}$_2$
of games
\mintinline{Coq}{G}$_1$, \mintinline{Coq}{G}$_2$
respectively.
%


